Analyzing the Components of Distributed Coevolutionary GAN Training

Distributed coevolutionary Generative Adversarial Network (GAN) training has empirically shown success in overcoming GAN training pathologies. This is mainly due to diversity maintenance in the populations of generators and discriminators during the training process. The method studied here coevolves sub-populations on each cell of a spatial grid organized into overlapping Moore neighborhoods. We investigate the impact on the performance of two algorithm components that influence the diversity during coevolution: the performance-based selection/replacement inside each sub-population and the communication through migration of solutions (networks) among overlapping neighborhoods. In experiments on MNIST dataset, we find that the combination of these two components provides the best generative models. In addition, migrating solutions without applying selection in the sub-populations achieves competitive results, while selection without communication between cells reduces performance.

==> background.tex <==
\section{Related Work}
\label{sec:background}

In this section we discuss work related to competitive coevolutionary
algorithms for minimax problems,  evolutionary computation
and GANs,  scaling evolutionary computation for machine
learning as well as GAN training.

\paragraph{Coevolutionary Algorithms for Minimax Problems}

%\CHECK{What is goal of this paragraph? Should we once again describe a competitive coev algorithm? We've provided some background in intro. What did we leave out that's important to mention? Let's not relate to GANS. Let's include: relative fitness functions (maybe, why?) and  traiing pathologies and EC solutions to them.}
%
%\CHECK{already said this in intro}Competitive coevolutionary algorithms have multiple adversarial populations (usually two) that simultaneously
%evolve~\cite{floreano2008bio,popovici2012coevolutionary}
%solutions against each other. 
%\CHECK{did not say this in intro, is it important for understanding Lipi?} They employ fitness functions that
%rate solutions relative to their \emph{adversaries}.  
%\CHECK{already said this in intro} Formally, these
%algorithms can be described with a minimax
%formulation~\cite{Herrmann1999Genetic,Ash2018Reckless,barbosa1999coevolutionary,Barbosa1997ACG}, which is a key characteristics they share with GANs.  
%\CHECK{already said this in intro}For example,
%mode collapse in GANs, which is when the generator collapses and produces a limited variety of samples, may arise from
%asymmetry~\cite{goodfellow2016nips} \TODO{Something new - Goodfellow attributes collapse to asymmetry see tutorial 3.2 and esp 3.2.5}. 
%\TODO{}To address this issue in
%competitive coevolution, \emph{asymmetric fitness evaluation} has been
%applied~\cite{jensen2003new,branke2008new,qiu2017new}.
%\TODO{we must finally define mode collapse and other pathologies} 
%\TODO{we must define asymmetry}
% see GAN Problems https://medium.com/@jonathan_hui/gan-why-it-is-so-hard-to-train-generative-advisory-networks-819a86b3750b
%
%Many GAN models suffer the following major problems:
%
%    Non-convergence: the model parameters oscillate, destabilize and never converge,
%    Mode collapse: the generator collapses which produces limited varieties of samples,
%    Diminished gradient: the discriminator gets too successful that the generator gradient vanishes and learns nothing,
%    Unbalance between the generator and discriminator causing overfitting, and
%    Highly sensitive to the hyperparameter selections.

Competitive coevolutionary algorithms have adversarial
populations (usually two) that simultaneously
evolve solutions against each other~\cite{floreano2008bio,popovici2012coevolutionary}. They employ fitness functions that rate a solution relative to its \emph{adversaries} and can sometimes be described as a zero-sum game or, more generally, a minimax optimization~\cite{Herrmann1999Genetic,Ash2018Reckless,barbosa1999coevolutionary,Barbosa1997ACG}. Without explicit remedies, they experience what we shall generally call \textit{pathologies} or \textit{limitations} in the form of non-convergent behavior, i.e. oscillations, and undesired but stable equilibria. Reasons offered for a limitation are usually accompanied by a general remedy and one or more methods to implement the remedy. For example, one reason offered for limitations is \textit{asymmetry}. \textit{Asymmetry} means that the fitness is not symmetrically applied to each of the adversaries.   \emph{Asymmetric fitness evaluation} has been applied as a remedy~\cite{jensen2003new,branke2008new,qiu2017new}.  It is, for example in GAN training, the use of Binary Cross Entropy as a loss metric for a generator and Mean Squared Error as a loss metric for a discriminator. As another example, \cite{cliff1995tracking} notes \emph{intransitive (cyclic)  superiority} and addresses it with more specific measures of fitness and genotypes to track the evolutionary dynamics.  

Watson and  Pollack~\cite{watson2001coevolutionary} used a collection of simple number games to illustrate three important coevolutionary
limitations namely, \textit{focusing}, which is a parallel to GAN mode collapse, \textit{relativism}, which is a parallel to GAN discriminator collapse, and \textit{loss of gradients}, which is a parallel to GAN vanishing
gradients.  A general reason offered for these limitations is that, despite the algorithm's stochasticity, the populations lack sufficient diversity to disrupt an oscillation or move the search away from an undesired equilibria.  Essentially, the population should serve as a source of novelty and a genotypically or phenotypically converged population fails in this respect.  One method of  preventing convergence is to supplement one or both populations with a memory that holds genotypes that have been previously visited. Memory has been implemented as a hall-of-fame~\cite{nolfi1998coevolving} or pareto archive~\cite{popovici2012coevolutionary}. Solutions in memory also serve as 
reference points with measuring the quality of a current solution and detecting a diminishing gradient.

Diversity has also been explicitly improved with competitive fitness
sharing~\cite{rosin1997new}, separation, e.g. a spatial topology~\cite{mitchell2006coevolutionary} or a spatial topology and temporal segregation~\cite{harper2014evolving}.  A spatial (2D toroidal) topology is an effective means of controlling
the mixing of adversarial populations in coevolutionary algorithms.
In a conventional setup, the members of populations are divided up on a grid of cells and overlapping neighborhoods for each cell are identified.   A neighborhood is defined by the cell itself and its adjacent
cells and specified by its size, $s$. Coevolution proceeds at each cell with populations drawn from the neighborhood. Compared to an algorithm where all members can or do interact with each other, this reduces the cost of
overall interaction from $\mathcal{O}(N^2)$ to $\mathcal{O}(Ns)$,
where $N$ is the size of each population. A Moore neighborhood with five cells 
(center and four cells respectively North, East, South and West) is
commonly used~\cite{Husbands1994Distributed}, see
Figure~\ref{fig:4x4-nhood}. With this design, each neighborhood can evolve in semi-isolation and
more diverse points in the search space are
explored~\cite{mitchell2006coevolutionary,williams2005investigating}.   It is this approach: spatial separation via an abstract cellular grid that contributes to our remedies for GAN training. Additionally, we explicitly improve diversity by using different loss functions during training.

\paragraph{Evolutionary Computation, Neural Nets and GANs}

Evolutionary Computation has been used to design neural networks
through neuroevolution~\cite{stanley2019designing}. NEAT and
HYPER-NEAT~\cite{stanley2002evolving,stanley2019designing} have been
updated to evolve deep network
architectures~\cite{costa2019coevolution}. In addition, population
based training of neural networks~\cite{jaderberg2017population} has
been investigated. Moreover, a combination of elements from deep
learning and artificial life demonstrated that coevolutionary neural
population models can simulate population dynamics, and that
evolutionary game theory can describe the
behavior~\cite{moran2018coevolutionary}.

One example of combining evolutionary computation and GANs is E-GAN. It 
evolves a population of three independent loss functions defined
according to three metrics (Jenson-Shannon Divergence --JSD, Least Squares -- LS distance, and a combination of JSD and Kullback-Leibler (KL) divergence)~\cite{wang2018evolutionary}. Each loss function is
independently used to train a generator from some starting condition,
over a batch. The generators produced by the loss functions are
evaluated by a single discriminator that returns a fitness value for
each generator. The best generator is then selected and training
continues, with the next training batch, and the three different loss
functions.  The use of different loss functions overcomes the
limitations of a single individual training objective and better
adapts the population to the evolution of the discriminator. The
results for problems  in the image domain have shown that E-GAN is able to obtain higher (better) inception scores,
while showing comparable stability when it converges. E-GAN relies on
the evolutionary population to introduce diversity into the training by its
different loss functions and it uses what can be described as evolutionary selection when updating the best generator of a batch.

\paragraph{Scaling Evolutionary Computing for Machine Learning}

One salient contribution of \horse is its scalability. There are other examples of scalable and large-scale evolutionary computation systems. One is EC-Star~\cite{hodjat2014maintenance} which runs on hundreds of desktop machines. In another, the team of ~\cite{salimans2017evolution} applied a simplified version of
Natural Evolution Strategies~\cite{wierstra2008natural} with a
novel communication strategy to a collection of reinforcement learning benchmark problems. Due to better parallelization over thousand
cores, they achieved fast training times (wall-clock time). They ran
their experiments on a computing cluster of $80$ machines and $1,440$
CPU cores~\cite{salimans2017evolution}. Another
team~\cite{clune2017uber} showed that deep convolutional networks with
over $4$ million parameters trained with genetic algorithms can also
reach competitive results. They employed a range of hundreds to
thousands of CPU cores (depending on availability). Deep networks have also been evolved on HPC~\cite{young2017evolving}. 

The bulk of attempts to improve GAN training have been designed to run on a single machine (or a single GPU). The advent of large-scale parallel
computation infrastructure prompts our interest in scaling them. 

\paragraph{Training GANs}

Robust GAN training is still an open research
topic~\cite{arora2017generalization}. Simple theoretical models
have been proposed to provide a better understanding of the
problem~\cite{li2017towards}. These will be used in Section~\ref{sec:TheoreticalWork} where we describe preliminary work that establishes that an evolutionary algorithm can ameliorate specific training problems. Several empirical
practices have been suggested to stabilize the
training~\cite{ganhacks}. Examples include hard-coded conditions to
decrease the optimizers' learning rate after a given number of
iterations~\cite{radford2015unsupervised}, ensemble
concepts~\cite{wang2016ensembles}or changing the generator's or
discriminator's
cost function~\cite{arjovsky2017wasserstein,mao2017least,nguyen2017dual,zhao2016energy}.  

The use of multiple generators and/or discriminators for improving robustness has also been studied.  This includes: training a cascade of GANs~\cite{wang2016ensembles};
sequentially training and adding new generators with boosting
techniques~\cite{tolstikhin2017adagan}; training multiple generators
and discriminators in parallel~\cite{jiwoong2016generative}; training
an array of discriminators specialized in a different low-dimensional
projection of the data~\cite{neyshabur2017stabilizing}; using several
adversarial ``local'' pairs of networks that are trained independently so
that a ``global'' supervising pair of networks can be trained against
them~\cite{chavdarova2018sgan}; and learning from a dynamic ensemble
of discriminators~\cite{mordido2018dropout}. 

Goodfellow in his 2014 paper describes basic GAN
training\cite{goodfellow2014generative}. Some training aspects can be
subtly changed, e.g. flipping a maximization objective to a
minimization objective to obtain a more informative gradient.  See
\cite{brownlee2019} for more details. There are many more loss
functions that have been formulated for GAN training, including
e.g. \cite{borji2019pros} which includes a large table of GAN
evaluation measures and \cite{shmelkov2018good,lucic2018gans} which
use two measures which approximate the recall (diversity) and
precision (quality of the image). There are also domain-specific
measures outside images, e.g. for text probability-based language
model metrics have been proposed~\cite{tevet2018evaluating}. 

 We  next  present our notation and formalize the goal of GAN training.   




==> conclusion.tex <==
\section{Conclusion \& Future Work}
\label{sec:conclusion}

In this paper, we have investigated how population diversity as
employed by spatial coevolutionary (in particular competitive)
algorithms as an option to enhance the performance of gradient-based
GAN training methods. We presented \horse, a framework that combines
the advantages of gradient-based optimization for GANs with those of
coevolutionary systems, and allows scaling over a distributed spatial
grid topology. Using a relatively small spatial grid is sufficient to
overcome the common limitations of GANs, due to the spatial grid and
asynchronous evaluation. The performance can improve with increased
grid size. In addition, \horse scales well up to the grid sizes
elaborated in the conducted experiments (i.e. a grid size of six by
six). We enhanced an existing spatial evolutionary GAN training
framework that promoted genomic diversity by probabilistically
choosing one of three loss functions. This method, called \SEGAN was
tested on the MNIST and CelebA data sets showed no drop in performance
and high diversity in label space, as well as on the TVD measure.

Future work will include the evaluation on more data sets and longer
training epochs. In addition, even better results may be achieved by
including improved GAN types like the recently introduced
WGAN~\cite{arjovsky2017wasserstein}. More heterogeneous cell
configurations, i.e. architectures and data slices can also be
explored. Furthermore, the constants in the computational complexity
of \horse could be reduced. Finally, other advancements in
evolutionary algorithms that can improve the robustness of GAN
training, e.g. temporal evolutionary training, need to be considered.


==> implementation.tex <==
\section{Methods implementation}
\label{sec:implementation}
This section summarizes the main aspects of the implementation of the three parallel methods studied in this research. 
\Lipi and \spagan are developed over open source MIT licensed. It is 
is written in \texttt{Python3} and uses \texttt{Pytorch}\footnote{Pythorch web site - \url{https://pytorch.org/}}.  
\texttt{Docker}\footnote{Docker web site - \url{https://www.docker.com/}} swarm and \texttt{docker-machine} is used to support distribution. 
The source is available from \url{https://github.com/mustang-gan/mustang/tree/master/mustang/src}. 

A master-client design model is used for communication. 
Clients are added by starting the application on more nodes, running pre-configured virtual machines, or with \texttt{Docker}. 

The master (or \emph{orchestrator}) is meant to control the whole training process. 
Its performs the following tasks: 
\begin{inparaenum}[\itshape 1)]
\item parsing the configuration, connecting to clients nodes, and transmiting the experiment configuration to all of them;
\item periodically checking client state, i.e. if the experiment has ended, or if the client may be not reachable anymore, unreachable clients can be ignored, or the entire experiment terminated;
\item gathering finished results, saving them to its disk, and ranking the final mixtures by their scores, e.g., FID. \end{inparaenum}

A modest computation power is required by the task overhead. 
The computation instances communicate with \textit{Hypertext Transfer Protocol} HTTP web services and exchange only relatively small amounts of data during the training process, 
it is possible to deploy multiple instances onto different machines and hence scale horizontally.

Each client node performs the computations of a sincle cell in the spatial grid. 
It starts by receiving the configuration parameters for the training process from the master. 
The client task can be summarized in three main steps:
\begin{inparaenum}[\itshape 1)]
	\item When a new experiment is requested, it parses the configuration file received and executes the specified training algorithm. It furthermore requests data from the neighboring cells each time the 	algorithm accesses the respective properties of the populations. 
If no experiment is running, the client runs in the background and listens for experiment requests on a specific port. 		
	\item It offers HTTP endpoints simultaneously to execute the training process. Other clients can also access these endpoints and request the current populations and optimizer parameters.
	\item The master actively monitors the clients and collects the
	results. After this, the client changes its state from \texttt{Busy}
	to \texttt{Idle} and waits for new experiment requests. 
\end{inparaenum}

==> methods.tex <==
\vspace{-0.1cm}
\section{Distributed GANs training methods}
\label{sec:methods}

In this study, we evaluate the impact of communication and selection
pressure on the performance and diversity of evolutionary GAN
training. Our belief is that too little diversity results in
convergence to pathological training states (as shown
by~\cite{schmiedlechner2018lipizzaner}) and too much diversity results
in divergence. The use of selection and communication is
one way of regulating the diversity.

We use varying degree of communication/isolation and selection
pressure through four distributed GAN training methods: 
%that return a generative model defined by an ensemble/mixture of generators called:
\pagan (Parallel GAN), \spagan (Spatial Parallel GAN), \nocommgan
(Isolated Coevolutionary GAN), and \Lipi. All these methods
train two populations (one of generators and one of discriminators).
Table~\ref{tab:features} summarizes the main features of these four algorithms. 

\begin{table}[!h]
\setlength{\tabcolsep}{1pt} % General space between cols (6pt standard)
\renewcommand{\arraystretch}{0.9} % General space between rows (1 standard)
  \centering
  \scriptsize
  %\vspace{-0.2cm}
  \caption{\small Key components of the GANs training methods.}
    %\vspace{-0.4cm}

  \label{tab:features}
\begin{tabular}{l|rrrr}
\toprule
\textbf{Feature} &  \textbf{\pagan} &  \textbf{\spagan} &  \textbf{\nocommgan} &   \textbf{\Lipi} \\
\midrule
\textbf{Definition of neighborhood (use of sub-populations)} & No & Yes & Yes & Yes\\
\textbf{Communication between sub-populations}  & No & Yes & No & Yes\\
\textbf{Application of selection/replacement operator}  & No & No & Yes & Yes\\
\bottomrule
\end{tabular}
  \vspace{-0.2cm}
\end{table}

The analyzed methods, first, adversarially train a population of generators $\mathbf{g}=\{g_1, ..., g_N\}$ and a population of discriminators $\mathbf{d}=\{d_1, ..., d_N\}$, one against the other (where $N$ is the size of the population). 
Second,  
%
%first, optimize the parameters (weights) of a
%population of generators $\mathbf{g}=\{g_1, ..., g_N\}$ and a
%population of discriminators $\mathbf{d}=\{d_1, ..., d_N\}$ one
%against the other, where $N$ is the size of the population; and
second, 
sub-populations of $\mathbf{g}$ ($\mathbf{g}^{k}$) are fused in
a mixture of generators according to given mixture weights ($w^k$) to
define the generative model~\cite{schmiedlechner2018lipizzaner}. Thus,
these distributed training methods address two different optimization
problems: training the GANs/optimizing networks weights and optimizing the mixture weights to maximize the quality of the generator ensemble.

\spagan, \nocommgan, and \Lipi address the robust
optimization/training of GANs by rising an arms-race between two
\textit{adversarial populations}, 
$\mathbf{g}=\{g_1, ..., g_N\}$ and $\mathbf{d}=\{d_1, ..., d_N\}$, where $N$ is the size of the populations. 
%
They
define sub-populations of $\mathbf{g}^{k}$ and $\mathbf{d}^{k}$ (we
drop the index for the sub-population when the context is clear) that
are trained one against the other in parallel. 
These sub-populations are defined according to the neighborhood relations in a toroidal grid
(see Section~\ref{sec:coev-gans}). These methods vary in the exchange of
information among the sub-populations during the training process and
the application or not of selection/replacement operator (see
Table~\ref{tab:features}). The use of populations are one source of
diversity, that has shown to be adequate to deal with some GAN
training pathologies~\cite{schmiedlechner2018towards,
  wang2019evolutionary, toutouh2019}.  
\pagan
basically takes advantage of computational resources available to
individually train $N$ GANs in parallel.
%
After training the populations, the $\mathbf{g}^{k}$ sub-populations are fused in a mixture of generators according to given mixture weights ($w^k$) to define the generative model~\cite{schmiedlechner2018lipizzaner}. 

Thus,
these distributed training methods address two different optimization
problems: training the GANs/optimizing networks weights and optimizing the $w^k$ mixture weights to maximize the quality of the generator ensemble.
%
This section, first, introduces the evolutionary method to
optimize the mixture weights that define the ensemble of generators;
second, it describes \pagan; finally, it presents the
spatially distributed GAN training algorithms. % (i.e., \spagan, \nocommgan, and \Lipi).


\subsection{Evolving Generator Mixture Weights}
\label{sec:weights-evolution} 

The generative models returned by the proposed methods consist on ensembles of $\mathbf{g}^{k} \in \mathbf{g}$ (a sub-population of
generators) of size $s\leq N$ and the mixture weight vector $\v{w}\ \R^{s}$,
where $w_i \in \v{w}$ represents the probability that a data point
drawn from $\mathbf{g}^{k}_i$ ($\sum_{w_i \in \v{w}^k} w_i = 1$).

%As the performance of $\mathbf{g}^{k}_i$ is optimized during the training presented bellow, 
For each cell ($k$), we optimize the accuracy of the generative model by evolving $\v{w}$.  Here, we evaluate GANs in creating images, thus, Fr\'echet Inception Distance (FID)~\cite{Martin2017GANs} score is used to asses the quality of the
generative models.  As the lower the better FID,
this is a minimization problem.  The problem is formulated in
Eq.~\ref{eq:mixture}.
%
\begin{equation}
\mathbf{g}^k, \v{w}^k =\argmin_{\mathbf{g}, \v{w}} \sum_{{g_i \in \mathbf{g} \\ w_i \in \v{w}}} w_i FID_{g_i}
\label{eq:mixture}
\end{equation}
 
We apply an Evolutionary Strategy to evolve $\v{w}$ to optimize the
weights. Specifically, an \texttt{ES}-(1+1) algorithm \cite{loshchilov2013surrogate} (see \alg~\ref{alg:mixture-ea}).

\setlength{\textfloatsep}{0pt}% Remove \textfloatsep
\begin{algorithm}
  \small
  \caption{\nameAlgMixture \newline%: \texttt{ES}-(1+1) to evolve mixture weights $\v{w}$. \newline
		\textbf{Input:}
		~$GT$~: Total generations, ~$\mu$~: Mutation rate , ~$\mathbf{g}$~: Sub-population of generators, $\v{w}$~: Mixture weights \newline
		\textbf{Return:}
		~$\v{w}$~: Mixture weights
	}\label{alg:mixture-ea}
	\begin{algorithmic}[1] 
	 \State $\v{w} \gets $ initializeWeights$()$ \Comment{Initialize mixture weights }
     \State $f \gets $ evaluateMixture($\v{w}, g$) \Comment{Evaluate generator mixture score}
	\For{generation} $\in [0,\dots, \text{GT}]$  \Comment{Loop over generations}
                \State $\v{w}' \gets $ mutate$(\v{w}, \mu)$ \Comment{Gaussian mutation of mixture weights }
		\State $f' \gets $ evaluateMixture($\v{w}', g$) \Comment{Evaluate generator mixture score}
                \If {$f' < f$} \Comment{ Replace if new mixture weights are better}
        		\State $\v{w} \gets \v{w}'$ \Comment{ Update mixture weights}
                \EndIf
         \EndFor
		\State \Return $\v{w}$
	\end{algorithmic}
\end{algorithm}

\subsection{\pagan GANs training}
\label{sec:pagan}

\pagan takes advantage of computational resources to individually
train $N$ pairs $g_i$-$d_i$ in parallel without any exchange of
information by applying the method presented
in~\cite{goodfellow2014generative}  (see \alg~\ref{alg:pagan}). When all the parallel GAN training finish,
the algorithm creates $N$ sub-populations of generators by applying a
\textit{bootstrapping} procedure that randomly selects $s \leq N$
generator from the entire population.  Then, ensembles are defined by
these sub-population of generators and their mixture weights computed
by applying \alg~\ref{alg:mixture-ea}.

\setlength{\textfloatsep}{0pt}% Remove \textfloatsep
\begin{algorithm}
	\small
	\caption{\nameAlgParallel \newline
	%: In pararllel, GANs are fully trained without exchanging any infomration with the other neighbors. At the end of the training process, a mixture weight vector $\mathbf{w}$ for each subpopulation is optimized to generate the mixture of generators. \\
		\textbf{Input:} ~T~: Total training epochs, ~$Z$~: Number of GANs, ~$\theta_{EA}$~: Parameters for \nameAlgMixture ,
		~$\theta_{Train}$~: Parameters for training the GANs, 
		~$s$~: Sub-population (bootstraps) size\newline
		\textbf{Return:}
		~$g$~: Sub-population of generators, ~$\mathbf{w}$~: Mixture weights
	}\label{alg:pagan}
	\begin{algorithmic}[1]
		
		\ParFor{$c \in E$} \Comment{Asynchronous parallel execution of all cells in grid}
		\State $g^* \gets$ TrainModels($\theta_{Train}, T$) \Comment{ GANs training~\cite{goodfellow2014generative}}
		\EndParFor
		\State $gs \gets$ \texttt{CreateNSubpopulations}($s,g^*$)\Comment{Bootstrapping to $g^*$ ($N$ times)}
		\ParFor{$g^i \in gs$} \Comment{Asynchronous parallel execution}
			\State $\mathbf{w}^i \gets$ \texttt{MixtureEA}($g^i, \theta_{EA}$)\Comment{Evolve mixture weights, \alg~\ref{alg:mixture-ea}} 
		\EndParFor
		\State $(g, \mathbf{w}) \gets$ \texttt{BestEnsemble}($g^*, \mathbf{w}^*$)\Comment{Get the ensemble with best FID} 
		\State \Return $(g, \mathbf{w})$ \Comment{Best mixture of generators} 
	\end{algorithmic}
\end{algorithm}


\subsection{Spatially distributed GANs training}
\label{sec:coev-gans}

\Lipi, \spagan, and \nocommgan represent different distributed
GAN training methods.  They define a toroidal grid in whose cells a
GAN is placed (called \textit{center}).  This allows the definition of
neighborhoods with sub-populations of $\mathbf{g}$ and of
$\mathbf{d}$. 
%In addition, it mitigates the quadratic computational
%complexity of the adversarial competitions applied by these training
%methods. 
The size of these sub-populations is denoted by $s$ ($s \leq N$).  Without loss of generality, we consider square grids of $m\times
m$, i.e., there are $m^2$ neighborhoods. In this study, a five-cell
Moore neighborhood ($s=5$) is used, i.e., the neighborhoods include
the cell itself (center) and the cells in the \textit{West},
\textit{North}, \textit{East}, and \textit{South} (see
Figure~\ref{fig:4x4-nhood}).

\begin{figure}[ht!]
  \includegraphics[width=1\linewidth]{figures/deep_neuroevolution_book_chapter.png}%{figures/4x4-nhood.pdf}
  \caption{Illustration of a 4$\times$4 grid (left) and the neighborhoods N$_{1,3}$ and N$_{1,1}$ with its sub-populations (right).}
  \label{fig:4x4-nhood}
\end{figure}

For the $k$-th neighborhood in the grid, we refer to the generator in
its center cell by $\mathbf{g}^{k,1}\subset \mathbf{g}$ and the set of
generators in the rest of the neighborhood cells by $\mathbf{g}^{k,2},
\ldots, \mathbf{g}^{k,s}$, respectively. Furthermore, we denote the
union of these generators by $\mathbf{g}^k = \cup^{s_n}_{i=1}
\mathbf{g}^{k,i} \subseteq \mathbf{g}$, which represents the $k$th
generator sub-population/neighborhood.

Each cell executes its own learning algorithm with its own learning
rate by applying an asynchronous parallel training.  \nocommgan
exchange information only to create the initial sub-populations.  Cells
in \spagan and \Lipi interact with the neighbors each training epoch.
This communication is carried out through the overlapping
neighborhoods in the spatial grid. Thus, each neighborhood gathers the
latest updated \textit{center} generator and discriminator of its
overlapping neighborhoods. 
Figure~\ref{fig:4x4-nhood}
illustrates some examples of the overlapping neighborhoods on a
\textit{4x4} toroidal grid. The updates in cell N$_{1,0}$ and N$_{1,2}$ will be communicated to the neighborhoods in the range of such a cell, e.g., N$_{1,1}$ and N$_{1,3}$.

%% TODO could we in a figure illustrate the communication differences?

%\begin{figure}[h!]
%  \includegraphics[trim={13.4cm 0 0 0},clip,width=0.7\linewidth]{figures/4x4-nhood.pdf}
%  \caption{Illustration of communication on the overlapping neighborhoods defined in the grid in Figure~\ref{fig:4x4-nhood}. The updates in cell N$_{3,2}$ will be communicated to the neighborhoods in the range of such a cell, e.g., N$_{0,2}$ and N$_{2,2}$.}
%  %. Propagation runs laterally and vertically}
%  \label{fig:4x4-nhood-comm}
%\end{figure}


\alg~\ref{alg:general-coev} summarizes the main steps of \Lipi,
\spagan, and \nocommgan.  It starts the parallel execution of the
training process in each cell.  First, the cell randomly initializes
single generator and discriminator models.  Then, the training process
consist on a loop: which comprises three main steps: \textit{i)}
gathering the GANs (neighbors) to update the neighborhood (not
performed by \nocommgan); \textit{ii)} updating the center according
to the training method (different for \Lipi, \spagan and \nocommgan);
and \textit{iii)} evolving the mixture weights by applying the
Evolutionary Strategy, ES-(1+1), shown in \alg~\ref{alg:mixture-ea}.
These three steps are repeated $T$ (training epochs) times.  
The returned generative model is the best performing neighborhood with its optimal mixture weights. 
 
\setlength{\textfloatsep}{0pt}% Remove \textfloatsep
\begin{algorithm}
	\small
	\caption{\nameAlgGrid \newline
	%:In parallel, for each cell, initialize settings then iterate over each generation. Each generation, retrieve neighbor cells to build generator and discriminator sub-populations, update the parameters of the generator and discriminator of the center of the cell trained with SGD (this process is the main difference between \spagan and \Lipi), and finally evolve weights for a neighborhood mixture model.\\
		\textbf{Input:} ~T~: Total training epochs, ~$E$~: Grid cells, ~$s$~: Neighborhood size,
		~$\theta_{EA}$~: Parameters for \nameAlgMixture, ~$\theta_{Train}$~: Parameters for training the models in each cell\newline
		\textbf{Return:}
		~$g$~: Neighborhood of generators, ~$\mathbf{w}$~: Mixture weights
	}\label{alg:general-coev}
	\begin{algorithmic}[1]
		
		\ParFor{$c \in E$} \Comment{Asynchronous parallel execution of all cells in grid}
		\State $n, \mathbf{w} \gets$ initializeNeighborhoodAndMixtureWeights($c, s$) \Comment{Uniform initialization of settings}
		\For{epoch} $\in [1,\dots, \text{T}]$ \Comment{Iterate over training epochs}
                \State $n \gets$ copyNeighbours($c, s$) \Comment{Gather neighbour networks} \label{alg:copy-neighboor}
		\State $n \gets$ TrainModels($n, \theta_{Train}$)\Comment{Update GANs weights} \label{alg:coev-training}
		\State $g \gets$ {getNeighborhoodGenerators}($n$)\Comment{Get the generators} 
		\State $\mathbf{w} \gets$ \texttt{MixtureEA}($\mathbf{w}, g, \theta_{EA}$)\Comment{Evolve mixture weights (\shortAlg~\ref{alg:mixture-ea})} \label{alg:coev-weights}
		\EndFor
		\EndParFor
		\State $(g, \mathbf{w}) \gets$ \texttt{BestEnsemble}($g^*, \mathbf{w}^*$)\Comment{Get the ensemble with best FID} 
		\State \Return $(g, \mathbf{w})$ \Comment{ Cell with best generator mixture } 
	\end{algorithmic}
\end{algorithm}

Now, we describe the three different methods to update the center GAN
of each cell, i.e. $\mathbf{g}^{k,1}$, $\mathbf{d}^{k,1}$,
(Line~\ref{alg:coev-training} of \alg~\ref{alg:general-coev}).

\subsubsection{\spagan (Spatial GAN Training)}
\label{sec:lipi-training}

The method applied by \spagan to train the models is described in
\alg~\ref{alg:spagan}.  It starts after gathering the latest version
of the GAN in the center of its neighbors ($\mathbf{g}^{i,1}$ and
$\mathbf{d}^{i,1}$) to build the sub-population $\mathbf{g}^k$ and
$\mathbf{d}^k$.  The training process is an iterative process applied
for each mini-batch of the training data.  This process has two main
stages: first, updating the learning hyperparameters by using
Gaussian-updates; and second, training the generator (discriminator)
in the center against a randomly chosen adversary.  The networks'
weights are updated according to the SGD by using the BCE loss (see
Eq.~\ref{eq:minmax-mut}).
 
\setlength{\textfloatsep}{0pt}% Remove \textfloatsep
\begin{algorithm}
	\small
	\caption{\nameAlgCellNoSelection \newline
	%:  Select a new neighborhood from the current one. Assign all models a loss function at random.  Each mini-batch train discriminators against a randomly drawn generator and generators against a randomly drawn discriminator, using SGD.   Evaluate all against each other, using min loss as value. Return this new neighborhood.\newline
		\textbf{Input:}
		~$\tau$~: Tournament size, ~$X$~: Input training dataset,
		~$\beta$~: Mutation probability, ~$n$~: Cell neighborhood sub-population, ~$M$~: Loss functions \newline
		\textbf{Return:}
		~$n$~: Cell neighborhood sub-population updated 
	}\label{alg:spagan}
	\begin{algorithmic}[1]
		\State $g_c, d_c \gets $ getCenter($\mathbf{g}, \mathbf{d}$) \Comment{ Get generator and discriminator at center }
		\State $\mathbf{B} \gets $ getMiniBatches($X$) \Comment{ Load mini-batches }
		\For{$B \in \mathbf{B}$} \Comment{Loop over batches}
		\State $n_{\delta} \gets$ mutateLearningRate($n_{\delta}, \beta$) \Comment{ Update learning rate} % with with Gaussian mutation }
		\State $d \gets$ getRandomOpponent($\mathbf{d}$) \Comment{ Get uniform random discriminator}
                %\State $g_c, d \gets \text{pick\_random}(M, g_c, d)$  \Comment{ Random draw of loss function for each generator and discriminator}
		\State $\nabla_{g} \gets$ computeGradient($g_c, d$) \Comment{ Compute gradient for center }
		\State $g_c \gets$ updateNN($g_c, \nabla_g, B$) \Comment{ Update with gradient }
		\State $g \gets$ getRandomOpponent($\mathbf{g}$) \Comment{ Get uniform random generator}
               % \State $g, d_c \gets \text{pick\_random}(M, g, d_c)$  \Comment{ Random draw of loss function for each generator and discriminator}
		\State $\nabla_{d} \gets$ computeGradient($d_c, g$) \Comment{ Compute gradient for center }
		\State $d_c \gets$ updateNN($d_c, \nabla_d, B$) \Comment{ Update with gradient }
		\EndFor		
		\State \Return $n$
	\end{algorithmic}
\end{algorithm}

\subsubsection{\nocommgan coevolutionary GAN training}
\label{sec:nocommgan-training}

\nocommgan applies coevolutionary training method to each
sub-population (neighborhood) in which each epoch is a generation of a generative loop (see \alg~\ref{alg:lipi}).  The
sub-populations are initialized at the beginning of the whole training
process with the unique exchange of information between neighbors
(after that there is not any migration among the cells).  The output of this method is the
sub-population $n$ with the updated \textit{center}.  We use
$\mathbf{g}$ and $\mathbf{d}$ to refer to $\mathbf{g}^k$ and
$\mathbf{d}^k$, respectively in \alg~\ref{alg:lipi}.
%
\nocommgan training coevolution is built on the following basis:
\textit{fitness evaluation}, \textit{selection and replacement}, and
\textit{reproduction based SGD}.

\sloppy
\paragraph{Fitness Evaluation}
The performance of a given generator (discriminator) is evaluated in
terms of the loss function $M$ when it is evaluated against the
adversaries discriminators (generators).  To accommodate this, in
\nocommgan, fitness $\calL$ of a model ($g_i\in \mathbf{g}$ or $d_j
\in \mathbf{d}$) is its average performance against all its
adversaries.

\paragraph{Selection and Replacement} 
Selection boosts fitter models over less fit ones.  First the
sub-populations with the updated copies of the neighbors are formed,
all GANs are evaluated, and selection is applied (lines from
\ref{alg:lipi-get-minibatch} to \ref{alg:lipi-select-center}).  Next,
when all GANs training is completed and all models are evaluated
again, \nocommgan replaces the least fit generator and discriminator
in the sub-populations with the fittest ones and sets them as the
\textit{center} of the cell (lines from \ref{alg:fit-eval-1.5} to
\ref{alg:replace-center}).  Here, we apply tournament selection.

\paragraph{SGD-based reproduction}
\label{sec:diversityPromotion}
To mutate the selected networks (i.e., update their parameters), a SGD-based method based on loss is applied (Section~\ref{sec:gan-training}). 
The center generator (discriminator) is evaluated against a randomly chosen
adversary from the sub-population of discriminators (generators) (lines
\ref{alg:lipi-rand-d} and \ref{alg:lipi-rand-g}, respectively).
Moreover, Gaussian-based
updates create new learning rate values $n_{\delta}$.  

\setlength{\textfloatsep}{0pt}% Remove \textfloatsep
\begin{algorithm}
	\small
	\caption{\nameAlgCell \\
	%:  Select a new neighborhood from the current one. Assign all models a loss function at random.  Each mini-batch train discriminators against a randomly drawn generator and generators against a randomly drawn discriminator, using SGD.   Evaluate all against each other, using min loss as value to choose best to replace worst and updating center. Return this new neighborhood.\newline
		\textbf{Input:}
		~$\tau$~: Tournament size, ~$X$~: Input training dataset,
		~$\beta$~: Mutation probability, ~$n$~: Cell neighborhood sub-population, ~$M$~: Loss functions \newline
		\textbf{Return:}
		~$n$~: Cell neighborhood sub-population updated
	}\label{alg:lipi}
	\begin{algorithmic}[1]
	\State $\mathbf{B} \gets $ getMiniBatches($X$) \Comment{ Load minibatches } \label{alg:lipi-get-minibatch}
	\State $B \gets $ getRandomMiniBatch($\mathbf{B}$) \Comment{ Get a minibatch to evaluate GANs}	
	\For{$g, d \in \mathbf{g} \times \mathbf{d}$} \Comment{Evaluate all GAN pairs}
		\State $\mathcal{L}_{g,d} \gets$ evaluate($g, d, B$) \Comment{ Evaluate GAN} \label{alg:fit-eval-1}
		\EndFor
	  \State $\mathbf{g}, \mathbf{d} \gets$ select($n, \tau$) \Comment{Select with min loss($\mathcal{L}$) as fitness } \label{alg:lipi-select-center}
		
		\For{$B \in \mathbf{B}$} \Comment{Loop over batches}
		\State $n_{\delta} \gets$ mutateLearningRate($n_{\delta}, \beta$) \Comment{ Update learning rate} % with with Gaussian mutation }
		\State $d \gets$ getRandomOpponent($\mathbf{d}$) \Comment{Get uniform random discriminator} \label{alg:lipi-rand-d}
		\For{$g \in \mathbf{g}$} \Comment{Evaluate generators and train with SGD}
                %\State $g, d \gets \text{pick\_random}(M, g, d)$  \Comment{ Random draw of loss function for each generator and discriminator} \label{alg:mut-line}
		\State $\nabla_{g} \gets$ computeGradient($g, d$) \Comment{ Compute gradient for $g$ }
		\State $g \gets$ updateNN($g, \nabla_g, B$) \Comment{ Update $g$ with gradient }
		\EndFor
		\State $g \gets$ getRandomOpponent($\mathbf{g}$) \Comment{ Get uniform random generator} \label{alg:lipi-rand-g}
		\For{$d \in \mathbf{d}$} \Comment{Evaluate discriminator and train with SGD}
                %\State $g, d \gets \text{pick\_random}(M, g, d)$  \Comment{ Random draw of loss function for each generator and discriminator} \label{alg:mut-line-2}
		\State $\nabla_{d} \gets$ computeGradient($d, g$) \Comment{ Compute gradient for $d$}
		\State $d \gets$ updateNN($d, \nabla_d, B$) \Comment{ Update $d$ with gradient }
		\EndFor
		\EndFor
		
		\For{$g, d \in \mathbf{g} \times \mathbf{d}$} \Comment{Evaluate all updated GAN pairs} \label{alg:fit-eval-1.5}
		\State $\mathcal{L}_{g,d} \gets$ evaluate($g, d, B$) \Comment{ Evaluate GAN} \label{alg:fit-eval-2}
		\EndFor
		\State $\mathcal{L}_{g} \gets average(\mathcal{L}_{\cdot, d})$ \Comment{ Fitness of $g$ is the average loss value ($\mathcal{L}$)}
		\State $\mathcal{L}_{d} \gets average(\mathcal{L}_{g,\cdot})$ \Comment{ Fitness of $d$ is the average loss value ($\mathcal{L}$)}    
		\State $n \gets$ replace($n, \mathbf{g}$) \Comment{ Replace the generator with worst loss}
		\State $n \gets$ replace($n, \mathbf{d}$) \Comment{ Replace the discriminator worst loss}
                \State $n \gets$ setCenterIndividuals($n$) \Comment{Best $g$ and $d$ are placed in the center} \label{alg:replace-center}
		\State \Return $n$
	\end{algorithmic}
\end{algorithm}



\subsubsection{\Lipi coevolutionary GAN training}
\label{sec:lipi-training}

\Lipi applies also the coevolutionary GAN training approach shown in
\alg~\ref{alg:lipi}~\cite{schmiedlechner2018lipizzaner}.  However, it
takes advantage of the toroidal grid to update $\mathbf{g}^k$ and
$\mathbf{d}^k$ copying the latest version of its neighbors after each
training epoch.  The output of this algorithm is the neighborhood with
the updated \textit{center} ($\mathbf{g}^{k,1}$ and
$\mathbf{d}^{k,1}$).


==> theoretical-models.tex <==
\section{Notation and Goal of GAN Training}\label{sec:notation}

We adopt the notation similar
to~\cite{arora2017generalization,li2017towards}.  Let $\calG=\{G_g, g
\in \calU\}$ and $\calD=\{D_d, d \in \calV\}$ denote the class of
generators and discriminators, where $G_g$ and $D_d$ are functions
parameterized by $g$ and $d$.  $\calU, \calV \subseteq \R^{p}$
represent the respective parameters space of the generators and
discriminators.  Finally, let $G_*$ be the target unknown distribution
to which we would like to fit our generative model.

\paragraph{GAN Training}
Formally, the goal of GAN training is to find parameters $g$ and $d$
in order to optimize the objective function
\begin{equation}
\label{eq:gan-def}
\min_{g\in \calU}\max_{d \in \calV} \calL(g,d)\;, \;\text{where} \nonumber
\end{equation}
\begin{equation}
\calL(g,d) = \E_{x\sim G_*}[\phi (D_d(x))] + \E_{x\sim G_g}[\phi(1-D_d(x))]\;,
\end{equation}
and $\phi:[0,1] \to \R$, is a concave \emph{measuring function}.  In
practice, we have access to a finite number of training samples $x_1,
\ldots, x_m \sim G_*$.  Therefore, an empirical version
$\frac{1}{m}\sum_{i=1}^{m} \phi(D_d(x_i))$ is used to estimate
$\E_{x\sim G_*}[\phi (D_d(x))]$. The same also holds for $G_g$.

These formalities allow us in the next section to next describe the preliminary work that motivated \horse.  

\section{Motivation for \horse's Design}\label{sec:TheoreticalWork}\label{sec:theor-gan-model}

This section presents key preliminary research we conducted which informed the design of \horse~\cite{schmiedlechner2018thesis,schmiedlechner2018towards}
To proceed we first used a simple theoretical problem from~\cite{li2017towards} where the generator set is characterized by two Gaussian means and the discriminator set has two pairs of parameters (enabling coverage of the generator's means).  % that exhibits degenerate training behavior in a typical GAN framework.  

Formally,
the generator set is defined as
\begin{equation}
\footnotesize
\label{eq:gens}
\calG = \bigg\{ \frac{1}{2}\normal(\mu_1,1) + \frac{1}{2} \normal(\mu_2, 1)\mid \vmu \in \R^2 \bigg\} \; .
\end{equation}
On the other hand, the discriminator set is expressed as follows.
\begin{equation}
\footnotesize
\label{eq:discs}
\calD = \{\I_{[\ell_1, r_1]} + \I_{[\ell_2, r_2]} \mid \vell, \vr \in\R^2 ~\mbox{s.t.}~\ell_1 \leq r_1 \leq \ell_2 \leq r_2 \} \; .
\end{equation}
Given a true distribution $G_{*}$ with parameters $\vmu^*$, the GAN objective of this simple problem can be written as
\begin{equation}
\footnotesize
\label{eq:mu-g}
\min_{\vmu} \max_{\vell, \vr} \calL(\vmu, \vell, \vr)\;, \; \text{where} \nonumber
\end{equation}
\begin{equation}
\footnotesize
\label{eq:loss}
\calL(\vmu, \vell, \vr) = \E_{x\sim G_{*}}[D_{\vell,\vr}(x)] + \E_{x\sim G_{\vmu}}[1 - D_{\vell, \vr}(x)]\;.
\end{equation}

Gradient-based training dynamics frequently exhibit mode and discriminator collapse when solving this problem. This assumes a conventional paradigm of single-generator and single-discriminator. The pathologies occur across empirical initializations of $\mu_1$ and $\mu_2$, e.g. see Figure~\ref{fig:mode-collapse}(a) where, for a set of training assumptions, very low likelihood of success, i.e. mode-collapse dynamics occur, when $\mu_1 = \mu_2$.  

We investigated alternatively training the generator set with a simple coevolutionary counterpart.  Our simple coevolutionary algorithm had a 10 member discriminator population and a 10 member generator populations. It used tournament selection, executed for 100 generations, and employed a simple Gaussian-based mutation on the four discriminator parameters: $\ell_1, r_1, \ell_2, r_2$ and/or the two generator parameters: $\mu_1$ and$ \mu_2$ : $\mathcal{N}(0,1)$, with a fixed step size of $1.0$. All models trained against all adversaries each generation. We examined whether the coevolutionary algorithm could avoid mode collapse and/or discriminator collapse.

%Figure~\ref{fig:gan-convergence} shows the convergence of the
%parameters $\ell_1,\ell_2, r_1, r_2, \mu_1, \mu_2$ using different
%variants of coevolutionary dynamics. Optimal discriminator and first
%order dynamics~\cite{li2017towards}, as well as symmetric and
%asymmetric fitness functions are shown. Note that the $\mu_1$ and
%$\mu_2$ under coevolutionary dynamics consistently converge to the
%true values $\mu^*_1$ and $\mu^*_2$, respectively. In addition, we
%investigated coevolutionary behavior for two scenarios that have been
%shown to be critical for traditional pure gradient-based GAN training
%methods \cite{arora2017gans, li2017towards}:

\emph{Mode collapse.} This is a frequently observed GAN failure, it
often occurs when attempting to learn models from highly complex
distributions, e.g. images of high visual quality
\cite{arora2017gans}. In this scenario, the generator is unable to
learn the full underlying distribution of the data, and attempts to
fool the discriminator by producing samples from a small part of this
distribution. Vice versa, the discriminator learns to distinguish real
and fake values by focusing on another part of the distribution --
which leads to the generator specializing on this area, and
furthermore to oscillating behavior.

In our experiment, we used the
same settings as \cite{li2017towards}, setting up problem scenarios where $\mu_1$ and $\mu_1$
were initialized to values in the interval of $[-10, 10]$, at step sizes of
$0.1$. Figure~\ref{fig:mode-collapse} shows the average success rate
with the given initialization values. We defined \emph{success} as the
ability to reach a distance less than $0.1$, between the best
generator of the last generation and the optimal generator
$G_*$~\cite{li2017towards}.  Coevolutionary GAN training was able to reliably solve all scenarios. It notably did so, 
even where conventional, gradient-based training fails, i.e. where $\mu_1=\mu_2$ we see a high success rate when comparing the
diagonal of Figure~\ref{fig:mode-collapse}~(b) to that of Figure~\ref{fig:mode-collapse}~(a).

\emph{Discriminator collapse.}  This describes the phenomenon where
the discriminator is stuck in a local minimum
\cite{li2017towards}. The local nature of gradient-based updates
complicates the escape from local minima without further
enhancements---a problem that global optimizers like evolutionary
algorithms handle better. For this scenario, the parameters of the generator population were fixed to
$\mu_1=-1, \mu_2=2.5$ during the whole evolutionary process and we investigated initializations of the 
discriminator parameters that pairwise were combinations of positive or negative values. This models dynamics that place a training algorithm's search point at different representative slopes in the fitness landscape.  Figure~\ref{fig:discriminator-collapse-progress}~(a) is a heat map of success rates showing how frequently the coevolutionary algorithm was successful. Notably for positive-negative, negative-positive and positive-positive parameter pairings the coevolutionary algorithm worked 100\% of the time. The lower left quadrant of the heat map (negative, negative) shows the coevolutionary algorithm worked close to 100\% of the time. Notably, a conventional GAN will \textit{frequently} collapse into the local minimum~(\cite{li2017towards}~Figure 2 (c)) from this initialization condition. Figure~\ref{fig:discriminator-collapse-progress}~(b) shows an initialization representative of this  quadrant, when all discriminator parameters are close to a local minimum.   Figure~\ref{fig:discriminator-collapse-progress}~(c) shows how a coevolutionary algorithm run escaped the local minima successfully. With more generations, the left bound asymptotically moves towards  $-\infty$. 

 \begin{figure}[tb]
   \subfloat[]{
     \includegraphics[width=0.48\textwidth]{figures/heatmap_optimal_madry.pdf}
     }
   \subfloat[]{
     \includegraphics[width=0.6\textwidth,clip]{figures/mode_collapse.pdf}
     }
   \caption{\small Heatmap of success probability for random
     \textbf{generator} ($\mu_1$ and $\mu_2$) initializations for (a)
     a variant of gradient-based dynamics (adapted
     from~\cite{li2017towards}) and (b) coevolutionary GAN training. For each square, the individuals of the generator
     population are initialized within the corresponding range.}
   \label{fig:mode-collapse}
 \end{figure}

 \begin{figure}[h]
     \includegraphics[width=1.0\textwidth,clip]{figures/discriminator-collapse-theoretical-model.pdf}
   \caption{\small (a) Heatmap of success probability for random
     \textbf{discriminator} ($\ell_1,r_1, \ell_2,r_2$) initializations
     for coevolutionary discriminator training.  The generator was not trained. The axes refer to
     initial values for both the left ($[\ell_1,r_1]$) and the
     right ($[\ell_2,r_2]$) bounds, leading to four different
     quadrants. Plots (b) and (c) show first and last generation of a coevolutionary
     trained GAN, initialized in a discriminator collapse setup, which
     corresponds to the bottom left quadrant of (a). In other words,
     for each square, the individuals of the discriminator population
     are initialized randomly such that the signs of their fitness
     values match those of the corresponding square.}
   \label{fig:discriminator-collapse-progress}
 \end{figure}

We further experimented with exchanging or removing parts of the competitive coevolutionary algorithm to understand their value. Using the theoretical and small problems, we determined that both the population property and the evolutionary selection with replacement mechanism are vital to success at avoiding collapses. We also found it possible to substitute gradient-based training for the Gaussian mutation when parameter training. When using gradient-based training, the aforementioned two coevolutionary algorithm features are sufficient to help a coevolutionary run succeed. Collapses do occur, but the populations, if large enough, rarely converge entirely on a collapsed model. In a timely manner, evolutionary selection pressure steps in to promote more resilient models. This change in parameter training method is important because, \textit{given gradient information is available, it is much more efficient to train with gradient information}. The final investigative detail that contributed  impetus to the design of \horse is the computational expense of the coevolutionary algorithm. Even with gradient-based training, competing one adversarial population against another each generation is $O(N^2)$.   Notably, a spatial configuration for a coevolutionary algorithm reduces this to $O(N)$. It is with these insights that we developed \horse.  We now proceed in the next section to describe \horse in detail.

